Hamiltonicity in random directed graphs is born resilient

Let $\{D_M\}_{M\geq 0}$ be the $n$-vertex random directed graph process, where $D_0$ is the empty directed graph on $n$ vertices, and subsequent directed graphs in the sequence are obtained by the addition of a new directed edge uniformly at random. For each $\varepsilon>0$, we show that, almost surely, any directed graph $D_M$ with minimum in- and out-degree at least 1 is not only Hamiltonian (as shown by Frieze), but remains Hamiltonian when edges are removed, as long as at most $(1/2-\varepsilon)$ of both the in- and out-edges incident to each vertex are removed. We say such a directed graph is $(1/2-\varepsilon)$-resiliently Hamiltonian. Furthermore, for each $\varepsilon>0$, we show that, almost surely, each directed graph $D_M$ in the sequence is not $(1/2+\varepsilon)$-resiliently Hamiltonian. This improves a result of Ferber, Nenadov, Noever, Peter and \v{S}kori\'{c}, who showed, for each $\varepsilon>0$, that the binomial random directed graph $D(n,p)$ is almost surely $(1/2-\varepsilon)$-resiliently Hamiltonian if $p=\omega(\log^8n/n)$.

==> picturedirhamres2.tex <==
\begin{tikzpicture}[scale=1.1]
\input{picturedirhamres1}
\draw (0,0) -- (1,0);
\draw (10,0) -- (11,0);

\foreach \x in {0,11}
{
\draw [fill] (\x,0) circle [radius=0.1cm];
}


\foreach \x in {0,10}
{
\draw ({\x+0.5},0) -- ({\x+0.4},0.1);
\draw ({\x+0.5},0) -- ({\x+0.4},-0.1);
\draw ({\x+0.6},0) -- ({\x+0.5},0.1);
\draw ({\x+0.6},0) -- ({\x+0.5},-0.1);
}
\


\foreach \x in {5}
{
\draw ({2*\x+0.5},-0.4) node {$S_1''$};
}

\foreach \x in {1}
{
\draw ({2*\x-1.5},-0.4) node {$S_1'$};
}

\foreach \y in {-1,-2,-3}
{
\draw (0,{-\y}) -- (11,{-\y});
}

\foreach \y in {-1,-2,-3}
{
\foreach \x in {0,11}
{
\draw [fill] (\x,{-\y}) circle [radius=0.1cm];
}
}

\foreach \y in {1,...,4}
{
\draw ({-0.3},{\y-1}) node {$s_\y$};
\draw ({11+0.3},{\y-1}) node {$t_\y$};
}


\foreach \y in {-1,-2,-3}
{
\draw (5.6,{-\y}) -- (5.5,{-\y-0.1});
\draw (5.6,{-\y}) -- (5.5,{-\y+0.1});
\draw (5.5,{-\y}) -- (5.4,{-\y-0.1});
\draw (5.5,{-\y}) -- (5.4,{-\y+0.1});
}
\foreach \y in {2,3,4}
\draw (5.5,{\y-1.3}) node {$S_\y$};


\draw (-0.5,3.5) -- (-0.5,-1.5) -- (11.5,-1.5) -- (11.5,3.5) -- (-0.5,3.5);

\draw (-1.1,1) node {$V(D)$};

\end{tikzpicture}

